Epsilon-shapes: characterizing, detecting and thickening thin features in geometric models

We focus on the analysis of planar shapes and solid objects having thin features and propose a new mathematical model to characterize them. Based on our model, that we call an epsilon-shape, we show how thin parts can be effectively and efficiently detected by an algorithm, and propose a novel approach to thicken these features while leaving all the other parts of the shape unchanged. When compared with state-of-the-art solutions, our proposal proves to be particularly flexible, efficient and stable, and does not require any unintuitive parameter to fine-tune the process. Furthermore, our method is able to detect thin features both in the object and in its complement, thus providing a useful tool to detect thin cavities and narrow channels. We discuss the importance of this kind of analysis in the design of robust structures and in the creation of geometry to be fabricated with modern additive manufacturing technology.

==> sections/intro.tex <==
% !TeX spellcheck = en_US
\section{Introduction}

==> sections/relatedworks.tex <==
% !TeX spellcheck = en_US

\section{Related Works}
\label{sec:related}

%
%
%\subsection{Shape Diameter Function \cite{Shapira:2008:CMP}} 
%
%\paragraph{Definition} Let $M$ be a manifold mesh surface defining a volumetric object. We define a scalar function on the surface $f_v : M \rightarrow \Re$ which we call the shape diameter function (SDF) as the neighborhood-diameter of the object at each point $P \in M$. On a smooth surface the exact diameter can be defined by the distance to the antipodal surface point using the 
%inward-normal direction. On a piecewise linear mesh, it is difficult to define the exact antipodal point. Moreover, we want to express the neighborhood shape diameter, which is different than the exact distance to the antipodal point.
%
%Given a point on the surface mesh we use a cone centered around its inward-normal direction (the opposite direction of its normal), and send several rays inside this cone to the other side of the mesh. For each such ray we check the normal at the point of intersection, and ignore intersections where the normal at the intersection points in the same direction as the point-of-origin (the same direction is defined as an angle difference less than 90$\degree$). This is done to remove false intersections with
%the ‘outside’ of the mesh. The SDF at a point is defined as the weighted  average of all rays lengths which fall within one standard deviation from the median of all lengths. The weights used are the inverse of the angle between the ray to the center of the cone. This is because rays with larger angles are more frequent, and therefore have smaller weights.
%
%\paragraph{Advantages} Invariant to rigid body transformations of the whole mesh. Furthermore, the SDF is oblivious to any deformation that does not alter the volumetric shape locally. This includes articulated character deformations, skeleton based movements or piecewise-rigid transformations. In essence, the SDF
%remains largely \textit{pose-oblivious}.
%
%\paragraph{Limitations} Using the SDF may have it’s limitation on 
%non-cylindrical parts of objects.
%
%%\subsection{Multiscale Area Projection Transform \cite{Giachetti:2012:RSD}} 
%
%\subsection{3D Minkowsky Sums \cite{Lien:2010:ASM}}
%
%\paragraph{Definition} The Minkowski sum of two polyhedra $P$ and $Q$ is defined as 
%
%\begin{equation}
%P \oplus Q = \{ p + q | p \in P, q \in Q \}.
%\label{eq:minkoqsky}
%\end{equation}
%
%Given two polyhedral models $P$ and $Q$ represented by their boundaries $\delta P$ and $\delta Q$, the boundary of their Minkowski sum $\delta(P \oplus Q) \ne \delta P \oplus \delta Q$. Therefore, computing the boundary-based representation of the Minkowski sums is more than applying Eq. \ref{eq:minkoqsky} to $P$ and $Q$. 
%
%\paragraph{Existing approaches} Despite the large volume of work, most methods can be categorized into one of the two main frameworks: divide-and-conquer and convolution. 
%
%In the \textit{divide-and-conquer} framework, the input models are 
%decomposed into components. Because computing the Minkowski sum of convex shapes is easier than non-convex shapes, convex decomposition (either surface or solid) is widely used. 
%
%The convolution of two shapes $P$ and $Q$, denoted as $P x Q$, is a set of line segments in 2-d or facets in 3-d that is generated by 'combining' the segments or the facets of $P$ and $Q$. 
%
%Alternatively, points have been used to represent the Minkowski sum boundary \cite{Tao:2008:CMS}. Representing the boundary using only points has many benefits. First of all, generating such points is easier than generating meshes and can be done in parallel and in multi-resolution fashion. Moreover, point-based representation can be generalized to higher dimensional motion planning problems. On the other hand, in \cite{Tao:2008:CMS}, a method is proposed to represent the boundary of the Minkowski sum approximately.
%
%\paragraph{Limitations} Computing the Minkowski sum of two polyhedra exactly has been shown difficult. Despite its fundamental role in many geometric problems in robotics, to he best of our knowledge, \todo{Da verificare CGAL \cite{CGAL}} no 3-d Minkowski sum  software for general polyhedra is available to the public. One of the main reasons is the difficulty of implementing the existing methods. Note that in  \cite{Lien:2010:ASM}, a new approach is proposed that is simple to implement  and can efficiently generate accurate Minkowski sum boundary. The author  declare that they intentionally sacrifice the exactness to maintain the simplicity.
%
%\subsection{Mathematical Morphology on meshes \cite{Lam:2011:USM}}
%
%\paragraph{Definitions}Mathematical morphology is based on set-theoretic concepts and its main operators, erosion and dilation, can be seen as operations between two sets. In image processing the sets are defined in $R^2$, but in general one can work in $R^n$. If $A$ is a set of points $p = (x_1,x_2,...,x_N)$ in Euclidean space $R^3$, then the
%binary set $A$ defines the surface and interior of a 3D object. Furthermore, if $B$ is also a set in $R^3$, $(B)_x$ denotes the translation of $B$ by $x$ and $\hat{B}$ is the reflection of $B$. The dilation of $A$ by $B$ is denoted by $A \oplus B$ and defined by
%
%\begin{equation}
%A \oplus B =  \{ x \in R_3 | (\hat{B})_x \cap A \ne \emptyset \}.
%\end{equation}
%
%Likewise, the erosion of $A$ by $B$ is denoted by $A \ominus B$ and defined by
%
%\begin{equation}
%A \ominus B = \{ x \in R^3 | (B)_x \in A \}.
%\end{equation}
%
%Boundary extraction in 2D can be defined by
%
%\begin{equation}
%\beta(A) = (A \oplus B) - (A \ominus B).
%\end{equation}
%
%In 3D, the boundary $\beta(A)$ is calculated on the dilated and eroded versions of object $A$ where $B$ is a sphere with radius
%$r$. In the limit case $r \downarrow 0$, $\beta(A)$ is the surface of $A$.
%
%\paragraph{Methods} There are a few important issues when applying mathematical morphology to 3D objects. One is associated with the type of representation: voxel or mesh. The voxel representation involves 3D arrays with, depending on the object’s resolution, very big dimensions, although the voxels themselves are binary: object vs. background. An advantage is that many algorithms from mathematical morphology have been developed for 2D image processing, and these can easily be adapted to 3D. Polygonal meshes, on the other hand, have a more complex data structure. After applying the erosion and dilation operators, the new meshes must be determined, very close vertices can be collapsed, and self-intersecting facets must be detected and removed.
%
%Dilations are obtained by displacing all vertices a distance $r$ (the radius) in the direction of the normal vector. Since
%normal vectors always point outside, this is $−r$ in the case of erosions. Both operators are applied in two distinct steps. The first one is intended to acquire the volumes of the objects after the erosion/dilation process. The second one is to keep the mesh 2-manifold.
%
%\subsection{Thickness Detection in 3D Printing \cite{Telea:2011:VBA}}
%The paper proposed a voxel-based method for the task of automated assessment of 3D printability. The method is mainly composed by the following steps:
%
%\begin{enumerate}
%	
%	\item Conversion of the input shape into a voxel grid, whose resolution exceeds that of the 3D printer. The output is a binary volume consisting of the shape $\Omega$ (foreground) and its complementary $\overline{\Omega} = R^3 / \Omega$ (background);
%	
%	\item \label{item:step_thin_detection} Thin region detection, by exploiting a top-hat transform. (\ref{item:step_thin_detection}a) Dilation of the erosion of $\Omega$ is performed by using a structuring element, that is a sphere having radius equal to the printer resolution; (\ref{item:step_thin_detection}b) Thin regions are obtained by the difference between the original input and its opening ( = dilation of erosion);
%	
%	\item Voxel classification into 4 categories: rump ($R$), thin ($T$), interface ($I$) and boundary ($B$). Classification is performed based on the following definitions:
%	\begin{equation}
%	R = \Omega / \Theta 
%	\end{equation}
%	where $\Theta$ is the set of detected thin regions;
%	
%	\begin{equation}
%		I = \{ x \in \Theta \mid \exists y \in n_6(x), y \in \Omega, y \notin \Theta \}
%	\end{equation}
%	
%	\begin{equation}
%		B = \{ x \in \Theta \mid \exists y \in n_6(x), y \in \overline{\Omega} \}
%	\end{equation}
%	where $n_6(x)$ is the set of 6 voxels connected to $x$.
%	
%	\begin{equation}
%		T = \Theta / (B \cup I)
%	\end{equation}
%	
%	\item Computation of printability metrics. Two metrics are proposed:
%	
%	\begin{itemize}
%		
%		\item \textbf{Area-based metric} marks large structures with small interfaces as more critical. Large structures are visually salient, and the smaller their interfaces are, the higher the chance is that the printer will not manage to render such connections or that such connections will be mechanically fragile. The area-based metric $\mu_A(C_i)$ of structure $C_i$ is computed as follows:
%		
%		\begin{equation}
%			\mu_A(C_i) = A_i^B / A_i^I
%		\end{equation} 
%		where $A_i^B = \sum_{}^{j}A_{ij}^B$ is the total boundary area of $C_i$, and $A_i^I = \sum_{}^{j}A_{ij}^I$ is the total interface area of $C_i$.
%		
%		The area-based metric fails detecting certain complex unprintable structures.
%		
%		\item \textbf{Geodesic length metric} measures the eccentricity of a structure. For a given component $C_i$, the geodesic length metric $\mu_G(C_i)$ is computed as 
%		
%		\begin{equation}
%			\mu_G(C_i) = \frac{\max_{x \in B, y \in I} \| (x \rightsquigarrow y) \|_2 }{\max_{x \in \delta I, y \in I} \| (x \rightsquigarrow y) \|_2 }
%		\end{equation} 
%		where $(x \rightsquigarrow y) \in \partial\Omega$ is a geodesic path on the shape $\partial\Omega = B \cup I$ between points $x$ and $y$.
%	
%	\end{itemize}
%
%\end{enumerate}
%
%\paragraph{Limitations} The proposed method can be used in a semi-automatic manner: the algorithm processes  set of shapes, identifies those with printability problems and shows them to the user for visual inspection. No automatic repairing is proposed.
%
%Voxelization resolution is currently the main limitation. Critical events smaller than one voxel is missed. Graphics cards are exploited to hold large voxel volumes and detect thin regions (the other operations are not computational expensive and are run on CPU). 
%
%\subsection{Thickening in 3D Printing \cite{Wang:2013:TFS}}
%Given a 2-manifold mesh surface $S$, a thickening operation generates a triangular mesh that represents the boundary surface $\partial H$ of a solid $H$, which is located at one side of $S$ and has a user-specified thickness $r$. Meanwhile, $\forall p \in S$ $(p \in R^3)$, the distance between $p$ and $\partial H$ must be zero.
%
%To solve this thickening problem, a new method is proposed that produces the boundary surface $\partial H$ in two steps. First, an implicit representation of the thickened solid $H$ is defined on an uniform grid, where each node stores a binary value to indicate whether the node is inside $H$. Then, a new partial surface reconstruction algorithm is investigated to generate the surface $\partial H$: the input surface $S$ is only modified to a new surface $\hat{S}$ by splitting the triangles on the boundary of $S$ if necessary, while other triangles are kept unchanged and the reconstructed surfaces for $\partial H$ are stitched to the boundary of $\hat{S}$. 
%
%In some more detail, the methods is built by the following steps:
%
%\begin{enumerate}
%	
%	\item Implicit solid representation by converting the input surface into an uniform grid;
%	
%	\item Evaluation of grid nodes. Each node stores its signed distance to the input surface $S$. Let $w$ be the width of the grid nodes, a node is defined as a \textit{valid} node if its distance is less than $\sqrt{3}w$. \textit{Candidate region} $\Omega \in R^3$ of valid grid nodes is defined as a set of points, where the distance of any point $q \in \Omega$ is less then (or equal to) $r + \sqrt{3}w$, where $r$ is the user-defined thickness. 
%	
%	Without loss of generality, we assume that there are $(2^l + 1) \times (2^l + 1) \times (2^l + 1)$ grid nodes to be assigned for the thickened solid $H(S)$. Starting from the bounding box $\phi$ of all these grid nodes, we recursively subdivide the boundary box into eight sub-boxes. For a sub-box, if the distance from the center $o$ of its circumsphere to the given surface $S$ is greater than $d + r + \sqrt{3}w$, the subdivision is stopped and all grid nodes in this sub-box are assigned as not belonging to the candidate region. Otherwise, the sub-box is further subdivided until a sub-box with only eight grid nodes is obtained, which cannot be further refined. 
%	
%	\item Partial surface reconstruction. The proposed approach is an extension of the \textit{dual contouring} algorithm.
%	
%	
%	
%\end{enumerate}
%
%\paragraph{Advantages} The input surface $S$ remains on the resultant model without introducing any approximation error. the model generated by the proposed method has nearly uniform thickness.
%
%\paragraph{Limitations} Evaluation of grid nodes is time consuming. Even if an optimization is applied, the computation of the signed distance field over the grid nodes still dominates the whole process. Multi-core CPUs are exploited to parallelize the computation.
%
%The input mesh is required to be intersection-free. If a self-intersected mesh is given, incorrect sign may be given to a grid node and an incorrect representation of the thickened solid is computed.
%
%
%
%\section{Other related works}
%
%\subsection{Trimesh offset}
%
%\begin{itemize}
%	\item \textit{Visualizing sphere-contacting areas on automobile parts for ECE inspection \cite{Inui:2015:VSC}} \\ In Section 2.2 of this paper, an overview of previous methods for offsetting 3D models is provided. \todo{Mi sembra che per lo più si utilizzino metodi basati su una grigliatura regolare dell'input -- metodi paralleli per velocizzare!} In this paper, a new offset-based method is proposed to automatically detect the possible sphere-contacting parts of an input shape. A polyhedral model that approximates the shape is given as an input, and the offset of the model is obtained as the Boolean union of the expanded shapes of all surface triangles. A triple-dexel representation of the 3D model is adopted to enable stable and precise Boolean union computations. A parallel approach is exploited to accelerate the computation. The possible sphere-contacting shape of the part surface is then extracted from the offset shape as a set of points or a set of polygons.
%
%	\item \textit{Offset Triangular Mesh Using the Multiple Normal Vectors of a Vertex \cite{Kim:2004:OTM}} \\ This paper introduces and illustrates the results of a new method for offsetting triangular mesh by moving all vertices along the multiple normal vectors of a vertex. The multiple normal vectors of a vertex are set the same as the normal vectors of the faces surrounding the vertex, while the two vectors with the smallest difference are joined repeatedly until the difference is smaller than allowance. Offsetting with the multiple normal vectors of a vertex does not create a gap or overlap at the smooth edges, thereby making the mesh size uniform and the computation time short. In addition, this offsetting method is accurate at the sharp edges because the vertices are moved to the normal directions of faces and joined by the blend surface. The method is also useful for rapid prototyping and tool path generation if the triangular mesh is tessellated part of the solid models with curved surfaces and sharp edges. \\ \textbf{Advantages} The method makes the mesh size uniform and the computation time is short. The method is precise and does not create gaps or overlaps at the smooth edges. No need to convert the input into a voxel grid or to a tetmesh. \\ \textbf{Limitations} The input triangular mesh needs to form a complete solid because the multiple normal vectors and the blend surfaces are calculated using topology.  
%
%\end{itemize}
%
%\subsection{Thickness Estimation on Trimeshes}
%
%\begin{itemize}
%	\item \textit{Robust Diameter-based Thickness Estimation of 3D Objects \cite{RollandNeviere:2013:RDB}}\\ 
%	\textbf{Abstract} We propose a robust thickness estimation approach for 3D objects based on the Shape Diameter Function (SDF). Our method first applies a modified strategy to estimate the local diameter with increased accuracy. We then compute a scale-dependent robust thickness estimate from a point cloud, constructed using this local diameter estimation and a variant of a robust distance function. The robustness of our method is benchmarked against several operations such as remeshing, geometric noise and artifacts common in triangle soups. The experimental results show a more stable local thickness estimation than the original SDF, and consistent segmentation results on defect-laden inputs.
%\end{itemize}
%
%\subsection{Thickness Estimation on Tetmeshes}
%
%Tetmeshes are used to represents biomedical 3D models. The following works propose a method to estimate the local thickness of tetmeshes. This method is based on volumetric Laplace-Beltrami opertor.
%
%\begin{itemize}
%	\item \textit{Impact of Early and Late Visual Deprivation on the Structure of the Corpus Callosum: A Study Combining 	Thickness Profile with Surface Tensor-Based Morphometry \cite{Shi:2015:IOE}} \\ \textbf{Data and program source code} developed in this manuscript 	are available under share-alike licenses upon request from N. Leporé and Y. Wang;
%	\item \textit{A Heat Kernel Based Cortical Thickness Estimation Algorithm \cite{Wang:2013:AHK}}.
%\end{itemize}
